Enabling Sparse Winograd Convolution by Native Pruning

Sparse methods and the use of Winograd convolutions are two orthogonal approaches, each of which significantly accelerates convolution computations in modern CNNs. Sparse Winograd merges these two and thus has the potential to offer a combined performance benefit. Nevertheless, training convolution layers so that the resulting Winograd kernels are sparse has not hitherto been very successful. By introducing a Winograd layer in place of a standard convolution layer, we can learn and prune Winograd coefficients "natively" and obtain sparsity level beyond 90% with only 0.1% accuracy loss with AlexNet on ImageNet dataset. Furthermore, we present a sparse Winograd convolution algorithm and implementation that exploits the sparsity, achieving up to 31.7 effective TFLOP/s in 32-bit precision on a latest Intel Xeon CPU, which corresponds to a 5.4x speedup over a state-of-the-art dense convolution implementation.

==> abstract.tex <==
\begin{abstract}

Sparse Winograd, as suggested by its name, combines a sparse method and the Winograd convolution algorithm, the two most successful approaches in speeding up convolution, and thus bears the promise of speeding up convolution over state-of-the-art. Nevertheless, efforts to realize sparse Winograd have not been very successful because of the challenges caused by the non-invertibility of Winograd transformation. We use a novel way to construct sparse Winograd by introducing a substitute for the convolution layer that we call, naturally,
the Winograd layer. This allows us to prune coefficients natively in the Winograd domain without involving Winograd transformations during training and pruning. Particularly, we define this Winograd layer, derive
the associated back propagation computations, design several train-and-prune
procedures, and implement a highly optimized sparse Winograd convolution for speeding up inference.
Our results achieve 90+\% sparsity in Winograd coefficients while maintaining
the original accuracy of AlexNet on ImageNet dataset.
On a latest Intel Xeon CPU, we show up to 5.4$\times$ speedup over dense direct
convolution with 31.7 effective 32-bit TFLOP/s in 3$\times$3 convolution layers
of AlexNet.

%Two recent and notable methods speed up, by several folds, convolution computations
%that are crucial to the performance of convolutional neural networks (CNNs).
%The first exploits the convolution kernels'
%sparsity that are obtained by suitable training and pruning procedures.
%The second uses transformation from ``spatial domain'' to the ``Winograd domain''
%where convolutions become element-wise multiplications. These two methods together
%naturally suggest potential for further performance
%improvement if the Winograd coefficients are sparse. Nevertheless, efforts to
%prune a network's Winograd coefficients via training and
%pruning procedures that work with both
%the spatial and Winograd coefficients simultaneously have not
%been very successful.
%%: They have not obtained Winograd coefficients with high sparsity
%%while preserving the original accuracy level exhibited by the network
%%when it is dense.
%We introduce a substitute for the convolution layer that we call, naturally,
%the Winograd layer. This allows us to prune coefficients natively in the Winograd domain without having to maintain a set of
%spatial coefficients. We define this Winograd layer, derive
%the associated back propagation computations, design several train-and-prune
%procedures, and designed a detailed performance model to quantify the potential speedup. Our results show more than 2$\times$ speedup over dense Winograd convolutions with achieved 90+\% sparsity in Winograd
%coefficients while maintaining the original accuracy of AlexNet on ImageNet dataset.
\end{abstract} 


==> arch_explained.tex <==
\begin{figure}
\includegraphics[width=3.2in]{arch-pictures.pdf}
\caption{
The red schematic on the top illustrates a traditional
convolution layer. This example takes the inputs ${\cal I}_j$, $j=1,2,3$,
and kernel parameters $w_{T,j}$, $j=1,2$, and produces the output
${\cal O}_j$, $j=1,2,3$.
The blue schematic on the bottom illustrates a corresponding
Winograd layer. Note that it takes three independent kernel
inputs $w_{F,j}$, $j=1,2,3$. Given any inputs ${\cal I}_j$,
the Winograd layer produces three outputs ${\cal O}_j$.
The standard Winograd-as-a-kernel implements a convolution layer
using the Winograd computation method, and is illustrated by the
green dotted line schematic. It takes the spatial convolution
parameters (two cofficients) $w_T$ and the input ${\cal I}$.
Internally, it applies the (non-invertible) transform to $w_T$
that yields $w_F = G w_T$, which is then used in the Winograd
computation. Consequently, the set of $w_F$ used here is at most
two dimensional, instead of the Winograd layer that can exploit
a three-dimensional input space for $w_F$.
}
\label{fig:architecture-explained}
\end{figure}


==> introduction.tex <==
\vspace{0.2cm}
\section{Introduction}\label{sec:introduction}

Convolution neural networks (CNN) have achieved undisputed success in many practical applications.
These deep neural networks typically contain multiple layers,
many (though not all) of which perform the namesake computation of convolution.
A convolution layer is an architecture whose connection between
an input and output tensor is via a number of convolution kernels,
and the basic arithmetic operations are that of multiply-accumulate.
Because over 90\%
of the computation during inference and
training of recent CNN designs is in convolutions~\citep{alexnet, googlenet}, different
compute kernels have been devised to speed up this core operation.
%GEMM-based kernels realize the convolutions as matrix multiplications and leverage
%optimization techniques familiar to matrix libraries implementors.
Recently, kernels
based on transform methods such as FFT~\citep{fft-cnn,fbfft} or
Winograd transformation~\citep{winograd1980arithmetic,winograd} have proved to be successful.
For the typical small convolution sizes (e.g., 3x3) that arise in CNNs, the Winograd-kernel approach
is more effective and has demonstrated more than twofold speed up
over well-implemented spatial convolution approaches.
%\jpark{A short discussion on sparse CNN with 3$\times$ speedups and that Winograd+sparse hasn't been successful?}.

The pursuit of faster convolution never stops. Besides the transform methods, sparse methods with pruned/compressed/sparse models demonstrate remarkable potential to accelerate convolutions while reducing model size~\citep{Brain_Damage:LeCun,scnn_lebedev,scnn}.
%The state of the art of spatial convolution implementation, however, has recently advanced noticeably.
For example, \cite{iclr17} demonstrated
that CNN with well pruned spatial convolution kernels
make convolution layers in inference as much as threefold faster provided the sparse
convolution operation is implemented competently. In principle, sparse methods and transform methods are orthogonal, and thus synergies between them can be leveraged to further accelerate convolutions. Particularly, applying sparse methods to Winograd convolution holds the most potential to achieve highest convolution speed for common convolution kernel sizes.

% This result suggests
%that CNN using Winograd kernel also has further performance
%improvement potential
%Nevertheless, pruning Winograd kernels is problematic:
%A pruned spatial convolution kernel does not lead to a pruned
%(sparsified) Winograd kernel. More important, one always has more
%Winograd coefficients than the corresponding spatial coefficients.
%In particular, the linear transform that maps spatial to Winograd
%coefficients is non-invertible. Thus any training method that needs
%to make use of both sets of coefficients in conjunction can only,
%if successful at all, arrive at sparse Winograd kernels that
%are in the range of the linear transform (i.e., very low sparsity in Winograd as shown in Section~\ref{subsec:sparsity_patterns}).

Nevertheless, pruning Winograd kernels poses challenges:
Firstly, even a well pruned spatial convolution kernel will always lead to a Winograd kernel with much reduced sparsity
%as shown in Section~\ref{subsec:sparsity_patterns},
because the Winograd transformation will introduce more non-zeros in the Winograd domain. More importantly, the linear transform that maps spatial to Winograd
parameters is non-invertible because the inverse transformation is an overdetermined system. Thus any training and pruning method that needs
to make use of both sets of parameters in conjunction will cause inconsistency, which in turn leads to major accuracy loss when achieving acceptable sparsity.% as shown in Section~\ref{subsec:sparsity_accuracy}.

\begin{figure}[t]
\includegraphics[width=\textwidth]{arch-pictures.pdf}%
\caption{\small
Schematic illustration for 1-D convolution and 1-D Winograd Convolution. The red schematic on the left illustrates a traditional
convolution layer. This example takes the inputs ${\cal I}_j$, $j=1,2,3$,
and kernel parameters $w_{T,j}$, $j=1,2$, and produces the output
${\cal O}_j$, $j=1,2$.
The blue schematic on the right illustrates a corresponding
Winograd layer. Note that it takes three independent kernel
inputs $w_{F,j}$, $j=1,2,3$. Given any inputs ${\cal I}_j$,
the Winograd layer produces two outputs ${\cal O}_j$.
The standard Winograd-as-a-kernel implements a convolution layer
using the Winograd computation method, and is illustrated by the
green dotted line schematic. It takes the spatial convolution
parameters (two cofficients) $w_T$ and the input ${\cal I}$.
Internally, it applies the (non-invertible) transform to $w_T$
that yields $w_F = G \times w_T$, which is then used in the Winograd
computation. Consequently, the set of $w_F$ used here is at most
two dimensional, instead of the Winograd layer that can exploit
a three-dimensional input space for $w_F$.
}
\label{fig:architecture-explained}
\end{figure}

In this paper, we show that pruning Winograd parameters becomes successful
% I replaced "possible" by successful. Pruning say in the Stanford report shows that
% it is possible, just that the result may not be outstanding.....
when we replace the convolution layer in question by
a Winograd layer, eliminating the need to use both the spatial
and Winograd parameters in conjunction. Figure~\ref{fig:architecture-explained} illustrates the architecture
of a Winograd layer using a simple 1D convolution of a 2-length spatial kernel
with 4-length input. The corresponding Winograd kernel is 3-length.
%The Winograd kernel approach is a computational method to realize the convolution
%architecture.
%When training a CNN, for example, computing the gradient of the loss function with respect to the
%convolution parameters is also dominated by convolution computations. This
%computation is sped up by using a Winograd kernel. The Winograd coefficients that emerge
%in this process are simply intermediate computed quantities.
%In contrast, we propose in this paper to define a Winograd
%layer as an architecture. The parameters of this layer play the role of the
%Winograd coefficients in the Winograd kernel, but are now ``first-class citizens'',
%and the parameters from the convolution kernel are no longer present.
%The architecture of the Winograd layer corresponds to computing a standard convolution
%layer using a Winograd kernel but have larger capacity: Given a specific convolution
%layer and the convolution parameters, we can construct a Winograd layer so that the two
%layers produce the same feature map output on the same feature map input; but the converse
%does not hold.
%

Replacing a convolution layer by a Winograd layer has several advantages. First, from a conceptual point of
view, this new layer architecture reflects directly the relationship between the key parameters
of the computation (which are the Winograd parameters) and the overall neural network.
Second, as alluded to earlier,
we have more Winograd than spatial parameters. Thus a Winograd layer in fact
has a larger capacity as we are no longer restricted to use only those Winograd
parameters that actually correspond to a set of spatial convolution parameters.
%
%which enables higher sparsity in Winograd parameters
%coefficients.
%\footnote{Winograd layer's larger capacity has other advantages such as achieving higher accuracy, which will be shown in Section~\ref{subsec:sparsity_accuracy} but this is not a focus of this paper.}.
%a Winograd layer has higher capacity. The reason is that
%the linear transform that maps convolution kernel parameters to Winograd parameters
%typically increase the parameters count. Using Winograd as a kernel in training
%therefore in effect more than double the memory cost (by working with both sets
%of parameters) without increasing the network's capacity. In contrast,
%the Winograd layer keeps only the Winograd parameters while exploiting the
%full capacity that these increased number of parameters offer.
Last but most important, steering of the training process such as pruning becomes
possible and straightforward. We emphasize that this is not the case if one
employs the spatial convolution layer:
the non-invertible mapping between convolution and
Winograd parameters is a major obstacle. While this obstacle may be overcome via approximation for small networks (LeNet) and datasets (MNIST) as reported in~\cite{sparse_winograd}, our experiments (Section~\ref{subsec:sparsity_accuracy}) show that approximation does not work for larger networks (AlexNet) and datasets (ImageNet).
%training -- an obstacle that seems not
%to be fully resolved there.
%\jpark{Somewhere around here, mention that high sparsity in time-domain does
%not result in high sparsity in Winograd domain for motivation.}

The main contributions of this paper are as follows.
\begin{enumerate}
\item We define and
advocate the use of the Winograd layer as an architecture. Details of
the forward and backward passes of this layer are derived and training
methods aim to prune are devised
(Sections~\ref{sec:winograd_layer_new}--\ref{sec:winograd_layer_sparsify}).
\item We design and implement a highly optimized sparse Winograd Convolution algorithm for fast inference by exploiting sparsity obtaining by pruning Winograd convolution layers (Section~\ref{sec:sparse_winograd_convolution}).
%\item We formulate a performance model of a Winograd layer whose
%parameters are possibly pruned (Section~\ref{sec:performance_model}).
%The model corroborates the expectation that pruned Winograd layers
%can outperform state-of-the-art convolution algorithms including both dense winograd convolution and spatial-domain sparse convolution.
\item We demonstrate the effectiveness of training and pruning with
the Winograd-layer architecture (Section~\ref{sec:results}). For instance, we prune AlexNet~\citep{alexnet} with its Winograd parameters pruned to more than 90\%, while maintaining its original accuracy.
This leads to more than 2$\times$ speedups over dense Winograd convolution, one of the fastest convolution algorithms to date~\citep{winograd}.
\end{enumerate}


==> performance_model.tex <==
\section{Inference Speed Projection of Sparse Winograd Layer}\label{sec:performance_model}

This section develops a performance model of sparse Winograd layers.
Our performance model demonstrates high speedup potential of combining Winograd
convolution with sparse computation, motivating sparse Winograd layer.
The performance model also
%informs "inform" is awkward as the object is usually a person (i.e. whom), eg
%I inform John that he has been fired, but here it informs
%"a range of sparsity"
pinpoints the range of sparsity where sparse Winograd
layer is most beneficial, thereby guiding the pruning process.
%We then discuss in which inference setup sparse Winograd layers will be particularly beneficial and its implication on future processor design.
%Since both Winograd convolution and sparse model significantly reduce the number of required floating point operations,
%it is important to consider if the memory bandwidth is the bottleneck.
%Suppose that a convolution layer performs $F$ floating-point operations (FLOPs hereafter), and transfers $B$ Bytes for input/output activations and parameters, respectively.
%Further suppose that the underlying hardware provides $F_{HW}$ FLOPs/second compute throughput and $B_{HW}$ Bytes/second memory bandwidth.
%The roofline performance model~\cite{roofline} calls $F/B$ {\it arithmetic intensity}, and the performance will be
%memory bandwidth bound if the arithmetic intensity is lower than that is provided by underlying hardware, $F_{HW}/B_{HW}$.
%In the recent Pascal-generation of Titan X, $F_{HW} \sim$10 single-precision TFLOP/s and $B_{HW} \sim$360 GB/s.
%Therefore, the Titan X needs at least 27 FLOPs per 1 Byte transferred from the memory not to be memory bandwidth bound.
%%The performance model cannot substitute the measurement of actual implementation on a real machine, but it is certainly more insightful than projection only based on FLOPs with additional benefit of separating out the factor of implementation quality.

Following the notations defined in Section~\ref{sec:winograd_layer_define},
consider a convolution layer with $C$ input channels each with a $H_i \times W_i$ image, $K$ output channels each with a $H_o \times W_o$ image, and
$CK$ convolution kernels each of size
$r\times s$. For simplicity, assume $H_i=W_i=H_o=W_o=H$ and $r=s$.
The number of floating point operations (FLOPs hereafter) in the baseline spatial convolution is
%the size of input/output activations in Bytes, the size of parameters in Bytes, are
\begin{align*}
F_\text{baseline} &= 2 C K H^2 r^2. %\\
%B_{act} &= 4(CH^2 + KH^2), B_{param\_base} = 4CKr^2,
\end{align*}
%respectively, assuming activations and parameters in 4 Bytes single-precision floating-point numbers.
%We focus on batch size 1, which is more challenging and interesting for settings with real-time constraints.
%We consider two cases when computing the Bytes transferred from memory: (1) activations
%between layers can stay in on-chip memory, where $B=B_{param}$ and (2) activations go off-chip, where $B=B_{act}+B_{param}$.
%This baseline convolution is compute intensive enough so that mostly compute bound in most recent hardwares,
%regardless of batch sizes.
%For example, 3$\times$3 and 5$\times$5 convolution layers in AlexNet and GoogLeNet have arithmetic intensity
%ranging 85--365 and 25--400 for batch size 1, and 350--700 and 150--580 for large batches, respectively.
%For example, 3$\times$3 and 5$\times$5 convolution layers in AlexNet and GoogLeNet have arithmetic intensity
%ranging 70--200 and 23--190, respectively, even in case (2) with more bandwidth pressure.
Unless otherwise noted, we count both multiplication and addition in the unit operation of convolution when calculating FLOPs, hence the coefficient of 2 in the equations.

Next, we consider sparse convolution (still in spatial domain)
with kernels whose density of non-zero parameters is $x$
(i.e. $100(1-x)$\% of parameters are zero).
\begin{align*}
F_\text{sparse} = 2 \alpha x CK H^2 r^2,
\end{align*}
where $\alpha$ denotes the overhead of sparse computation.
In the ideal case of $\alpha=1$, we will get speedups
inversely proportional to $x$.
In practice,
there is typically an overhead associated with processing using
sparse representations (e.g., $\alpha \approx 3$ has been observed on CPUs~\cite{iclr17}).

In Winograd-based convolution with $m\times m$ tiling,
\begin{align*}
F_\text{winograd} =
\mathbf{2} \left(2Cp^2 + \mathbf{CKp} + Km(m + p)\right) \mathbf{p\left(\frac{H}{m} \right)^2},
%, \\
%B&_{act\_winograd} = B_{act\_base}, \\
%B&_{param\_winograd} = 4CK(r+m-1)^2.
\end{align*}
where $p=r+m-1$.
The boldfaced term corresponds to the element-wise products in Equation~\ref{eqn:conv-winograd} and dominates the total computation when $C$ and $K$ are large enough.
The other terms correspond to the transformation of input and output activations between Winograd and spatial domains
(multiplications with matrices $A_1$, $A_2$, $B_1$, and $B_2$).
For simplicity, we assume not to take advantage of many -1, 0, and 1 appearing in these matrices.
%In case (2), Winograd convolution reduces the arithmetic intensity of 3$\times$3 and 5$\times$5 convolution layers in AlexNet to 9--34, which is neither completely compute nor bandwidth bound.

Finally, we consider sparse Winograd model with non-zero density $x$.
\begin{align*}
F&_\text{sparse\_winograd} =
\mathbf{2}\left(2Cp^2 + \mathbf{\alpha xCKp} + Km(m + p) \right) \mathbf{p\left(\frac{H}{m} \right)^2},% \\
%B&_{act\_sparse\_winograd} = B_{act\_base}, \\
%B&_{param\_sparse\_winograd} = \beta x 4CK(r+m-1)^2,
\end{align*}
%where $\alpha$ and $\beta$ denote the compute and storage overheads of sparse representations, respectively.
%, and $\beta$ is typically 2 in the popular compressed sparse row (CSR) representation.
where the boldfaced term for element-wise products with sparsified parameters is multiplied with $\alpha x$ times,
while the other terms for transformation remain the same.\footnote{
If the parameters associated with a given input or output channels are all zero, we can also reduce the computation
associated with transformation, but we find such channels whose associated filters are all zeros are not frequent.
There is a method to actively encourage group-wise sparsity with group Lasso regularization~\cite{scnn_lebedev,sscnn}, but
such method results in lower sparsity (typically $\sim$50\%) than methods for element-wise sparsity (typically $\sim$90\%)
%%when looking for  very small accuracy drop from sparsification.
%..peter's comments: need a "subject" for "looking for"..who is looking for this?
to maintain the accuracy.}

\begin{figure}[t]
%\label{fig:performance_model}
\centering
\subfigure[b][conv2]{
\centering
\includegraphics[width=.45\columnwidth]{conv2_perf_projection_cropped.pdf}
}
\subfigure[b][conv3]{
\centering
\includegraphics[width=.45\columnwidth]{conv3_perf_projection_cropped.pdf}
}
%\label{fig:performance_model}
\caption{Projected inference speedups of {\tt conv2} and {\tt conv3} of AlexNet
with varying sparsity.
}
\label{fig:performance_model}
\end{figure}

\definecolor{Gray}{gray}{.9}
\begin{table*}
\caption{The sparsity, projected inference speedups, and top-1 test accuracy of 3$\times$3 and 5$\times$5 convolution layers of AlexNet resulted from different pruning methods. The accuracy of the original AlexNet is 57.4\%.
{\tt Training Domain}: the domain where we compute derivatives and optimize using SGD.
{\tt Pruned Domain}: the target domain where we apply regularization and thresholding to increase the sparsity, which is also the domain where we measure sparsity.
{\tt Method A}: the method of training and pruning directly in Winograd domain described in Sections~\ref{sec:winograd_layer_define}--\ref{sec:winograd_layer_sparsify}.
{\tt B}: the method using spatial and Winograd parameters in conjunction similarly to \cite{sparse_winograd}.
{\tt B1} and {\tt B2} are with different hyper-parameters, {\tt B1} to match the sparsity with method A and {\tt B2} to match the accuracy.
{\tt C}: spatial domain pruning results from \cite{iclr17}.
}
\label{tab:results}
\centering
\small
\begin{tabular}{c c c | c | c c c c | c c c c }
\\
\hline
                         & Training                  & Pruned                     & Top-1    & \multicolumn{4}{c|}{Sparsity of Convolution Layers} & \multicolumn{4}{c}{Projected Inference Speedups} \\
\multirow{-2}{*}{Method} & Domain                    & Domain                     & Accuracy & {\tt conv2} & {\tt 3} & {\tt 4} & {\tt 5}           & {\tt conv2}     & {\tt 3}     & {\tt 4}     & {\tt 5} \\
\hline
A (Ours)                 & Winograd                  & Winograd                   & 57.3\%   & 90.6\%      & 95.8\%  & 94.3\%  & 93.9\%            & 5.2$\times$ & 9.4$\times$ & 6.0$\times$ & 4.8$\times$ \\
\hline
B1                       &                           &                            & 49.3\%   & 92.8\%      & 94.2\%  & 93.2\%  & 91.1\%            & 5.5$\times$ & 8.0$\times$ & 5.6$\times$ & 4.2$\times$ \\
B2                       & \multirow{-2}{*}{Spatial} & \multirow{-2}{*}{Winograd} & 57.3\%   & 54.1\%      & 67.5\%  & 62.4\%  & 60.2\%            & 2.6$\times$ & 2.3$\times$ & 1.9$\times$ & 1.7$\times$ \\
\hline
C                        & Spatial                   & Spatial                    & 57.4\%   & 85.6\%      & 93.1\%  & 91.8\%  & 88.5\%            & 2.3$\times$ & 4.8$\times$ & 4.1$\times$ & 2.9$\times$ \\
\hline
\end{tabular}
\end{table*}

Using the performance model, Figure~\ref{fig:performance_model} plots the projected inference speedups of the 3$\times$3 and 5$\times$5 convolution layers of
AlexNet for the range of sparsity obtainable with our training method that will be presented in the following section\footnote{
When applying compute reduction techniques such as Winograd convolution and sparse convolution, it is important to check if
performance is not memory bandwidth bound. We check the performance is indeed not memory bandwidth bound for the sparsity range plotted in Figure~\ref{fig:performance_model}, assuming 10 FLOP/Byte
ratio of compute throughput to memory bandwidth provided by the underlying hardware.
}.
For a very high sparsity like $x \leq 0.05$, sparse convolution in spatial domain is projected to provide higher speedups than
sparse Winograd convolution.
This is because the transformation part of sparse Winograd convolution does not benefit from sparsity.
However, in reality the achievable sparsity without accuracy loss is higher in Winograd domain than in spatial domain. Therefore, for the range of sparsity we can actually obtain without accuracy loss, sparse Winograd convolution has higher projected speedups than sparse spatial convolution as to be shown in Section~\ref{sec:results}.

Our performance model can be used to determine whether sparse Winograd convolution will be beneficial for a given CNN model and underlying hardware.
In Figure~\ref{fig:performance_model}, Sparse Winograd convolution is projected to outperform dense Winograd with sparsity higher than 67\% (i.e. $x<1/3$) because we assume the overhead of sparse computation, $\alpha$, to be 3.
If a convolution layer does not yield a higher sparsity, it is not useful to attempt to prune that layer. In fact, this is usually the case for the first convolution layer.
If a processor architecture has smaller overhead, sparse Winograd convolution can benefit at a wider range of sparsity.
%For example, without accuracy drop, {\tt conv2-5} of AlexNet can have 85-93\% sparsity ($0.07 < x < 0.15$) in spatial domain and
%91-96\% sparsity ($0.09 < x < 0.04$) in Winograd domain.

\iffalse
Consider $N$ output channels, $C$ input channels each with $H_i\times W_i$, $r\times s$ convolutions, and $m\times m$ Winograd tile size.
For simplicity, assume $H = W$ and $r = s$.

The number of floating point operations in the baseline dense convolution is $2NCH^2 r^2$.

The number of floating point operations in the Winograd convolution is $2C\left \lceil{\frac{H+r-1}{m}}\right \rceil^2 (r+m-1)^4 + 2NC\left \lceil{\frac{H+r-1}{m}}\right \rceil^2(r+m-1)^2 + 2N\left \lceil{\frac{H+r-1}{m}}\right \rceil^2 (r+m-1)^2 m^2$. The first term is for transforming the input tensor and the last term is for inverse-transforming the output tensor. The second term is for element-wise product of the transformed input tensor and weight tensor (main part of Winograd convolution), and this is the term sparsity helps. Note that $\left \lceil{\frac{H+r-1}{m}}\right \rceil^2$ is the number of Winograd tiles per channel.

For small batch sizes, the activation data generated by the previous layer will stay in on-chip caches. Therefore, the off-chip memory bandwidth is mainly used for accessing the weight tensor. Let $F$ be the peak compute capability of the processor (in FLOP/s), $B$ be the memory bandwidth (in B/s), $x$ be the density of weight tensor after pruning, $\alpha$ be the compute overhead of sparse computation, and $\beta$ be the storage overhead of sparse format. Then, the performance can be projected as in Figure~\ref{fig:performance_model}.

\begin{figure*}
\begin{align*}
& t_{dense} = max\left(\frac{2NCH^2 r^2}{F}, \frac{4NCr^2}{B}\right) \\
& t_{sparse} = max\left(\frac{\alpha x 2NCH^2 r^2}{F}, \frac{\beta x 4NCr^2}{B}\right) \\
& t_{Winograd} = \\
& \ max\left(\frac{2\left \lceil{\frac{H+r-1}{m}}\right\rceil (r+m-1)^2 (C(r+m-1)^2+Nm^2) + 2NC\left\lceil{\frac{H+r-1}{m}}\right\rceil^2(r+m-1)^2}{F}, \frac{4NC(r+m-1)^2}{B}\right) \\
& t_{Winograd\_sparse} = \\
& \ max\left(\frac{2\left \lceil{\frac{H+r-1}{m}}\right\rceil (r+m-1)^2 (C(r+m-1)^2+Nm^2) + \alpha x2NC\left\lceil{\frac{H+r-1}{m}}\right\rceil^2(r+m-1)^2}{F}, \frac{\beta x4NC(r+m-1)^2}{B}\right)
\end{align*}
%\label{fig:performance_model}
\caption{Performance Model}
\end{figure*}
\fi


==> previous_texts.tex <==
Consider $F(m\times m, r\times r)$ Winograd transformation and
suppose input tensor $\bm{\mathcal{I}} \in \mathbb{R}^{C\times H_i \times W_i}$, weight tensor in Winograd domain $\bm{\hat{\mathcal{G}}} \in \mathbb{R}^{N\times C\times (m+r-1)\times (m+r-1)}$, and output tensor $\bm{\mathcal{O}} \in \mathbb{R}^{N\times H_o \times W_o}$.
Since Winograd transformation is applied to tile by tile, we rearrange the tensor elements tile by tile.
$F(m\times m, r\times r)$ Winograd algorithm is applied to $(m+r-1)\times(m+r-1)$ image tile with $(r-1)$ elements of overlap with neighboring tiles.
When we rearrange the input tensor tile by tile, we duplicate the elements in the overlaps (somewhat similar to lowering applied to input tensor of time-domain convolution layer in Caffe but with much less duplicates).

After the rearrangement, we have $\bm{\mathcal{I}'} \in \mathbb{R}^{C\times (H_o W_o/m^2) \times (m+r-1)^2}$ and $\bm{\mathcal{O}'} \in \mathbb{R}^{N\times (H_o W_o/m^2)\times m^2}$.

Winograd transformation to compute $n$th output channel, $i$th tile is
%\[
%\bm{\mathcal{O}'}(n,i,:,:) = A^\intercal \left[\sum_{c}\bm{\hat{\mathcal{G}}}(n,c,:,:)\odot (B^\intercal \bm{\mathcal{I}'}(c,i,:,:) B) \right] A
%\]
\[
\bm{\mathcal{O}'}(n,i,:) = (A\otimes A)^\intercal \sum_c\left[ \bm{\hat{\mathcal{G}}}(n,c,:)\odot \left((B\otimes B)^\intercal \bm{\mathcal{I}'}(c,i,:)\right)\right]
\]

We also introduce intermediate tensors, $\bm{\mathcal{W}} \in \mathbb{R}^{C\times (H_o W_o/m^2)\times (m+r-1)^2}$ and $\bm{\mathcal{Z}} \in \mathbb{R}^{N\times (H_o W_o/m^2)\times (m+r-1)^2}$ such that

\[
\bm{\mathcal{W}}(c,i,:)=(B\otimes B)^\intercal \bm{\mathcal{I}'}(c,i,:)
\]
\[
\bm{\mathcal{Z}}(n,i,:)=\sum_c \left[\bm{\mathcal{G}}(n,c,:)\odot \bm{\mathcal{W}}(c,i,:) \right],\text{ or }\bm{\mathcal{Z}}(:,:,j)=\bm{\hat{\mathcal{G}}}(:,:,j) \bm{\mathcal{W}}(:,:,j)
\]
\[
\bm{\mathcal{O}'}(n,i,:) = (A\otimes A)^\intercal \bm{\mathcal{Z}}(n,i,:)
\]

Now, we apply the chain rule.

\begin{align}
\frac{\partial L}{\partial \bm{\mathcal{Z}}}(n,i,:) &= (A\otimes A) \frac{\partial L}{\partial \bm{\mathcal{O}'}}(n,i,:) \\
\frac{\partial L}{\partial \bm{\mathcal{W}}}(:,:,j) &= \bm{\hat{\mathcal{G}}}(:,:,j)^\intercal \frac{\partial L}{\partial \bm{\mathcal{Z}}}(:,:,j)\\
\frac{\partial L}{\partial \bm{\hat{\mathcal{G}}}}(:,:,j) &= \frac{\partial L}{\partial \bm{\mathcal{Z}}}(:,:,j) \bm{\mathcal{W}}(:,:,j)^\intercal \\
\frac{\partial L}{\partial \bm{\mathcal{I}'}}(c,i,:) &= (B \otimes B) \frac{\partial L}{\partial \bm{\mathcal{W}}}(c,i,:)
\end{align}

\section{Background Notes (by Peter)}
These notes are more for the Peter's benefit than anything else. Just to do things step by step.

A simple layer in Caffe seems to be $(X, W) \rightarrow Y$ where $X$ is the input (bottom), $W$ are parameters, and $Y$
is the output (top). When the layer is asked to do a forward step, it simply use $X$ and $W$ to produce $Y$. When
a backward step is asked for, I believe the following:
\begin{itemize}
\item $\frac{\partial L}{\partial Y}$ is known (available), that is already computed.
\item The backward step should compute $\frac{\partial L}{\partial X}$, using the values of $\frac{\partial L}{\partial Y}$
      as well as possibly the values of the parameters $W$.
\item The backward step should also produce $\frac{\partial L}{\partial W}$ based on $\frac{\partial L}{\partial Y}$
      and the input values $X$.
\end{itemize}
Here, I will consider two cases of how $Y$ is produced by $X$ and $W$ and work out the layer computation.
      
Consider the simple case $Y = W X$ where

\begin{tabular}{l l l}
$X$	& is & $N$-by-1  \\
$Y$ & is & $M$-by-1  \\
$W$ & is & $M$-by-$N$
\end{tabular}

The forward step is trivial. For the backward step
\begin{itemize}
\item $\frac{\partial L}{\partial X} = W^T \frac{\partial L}{\partial Y}$
\item $\frac{\partial L}{\partial W}(m,n) = \frac{\partial L}{\partial Y_m} X_n$, in other words
      $\frac{\partial L}{\partial W} = \frac{\partial L}{\partial Y} X^T$.
\end{itemize}

Next consider the case $Y = W X$ where $Y$ and $X$ are 2 dimensional.

\begin{tabular}{l l l}
$X$	& is & $N$-by-$K$  \\
$Y$ & is & $M$-by-$K$  \\
$W$ & is & $M$-by-$N$
\end{tabular}

Here each column of $Y$ is transformed by the same linear transformation applied to a corresponding column of $X$. 
The forward step is trivial. The backward step requires just a little more care to get correct.
\begin{itemize}
\item $\frac{\partial L}{\partial X}(:,k) = W^T \frac{\partial L}{\partial Y}(:,k)$
\item Consider the partial derivative of $L$ with respect to $W_{m,n}$. $W_{m,n}$ affects the entire $m$-th
      row of $Y$: $Y_{m,k} = W_{m,n} X_{n,k} + \hbox{terms unrelated to $W_{m,n}$}$. Therefore
      $$
      \frac{\partial L}{\partial W_{m,n}} = \sum_k \frac{\partial L}{\partial Y_{m,k}} \,
                                                   \frac{\partial Y_{m,k}}{\partial W_{m,n}}
                                          = \sum_k \frac{\partial L}{\partial Y_{m,k}} \,
                                                   X_{n,k}
      $$
      In other words, $\frac{\partial L}{\partial W} = \frac{\partial L}{\partial Y} X^T$.
\end{itemize}

\section{Back Propagation for Winograd Layer}
This is basically a re-derivation of the first section based on its characterization of how the layer is defined.
Here, the layer is $({\cal I'}, \hat{\cal G}) \rightarrow {\cal O'}$ where ${\cal I'}$ is the input
data, $\hat{{\cal G}}$ is the parameter, and ${\cal O'}$ is the output. The input/output is related by the following

\begin{enumerate}
\item ${\cal W}(c,i,:) = {\cal B}^T {\cal I'}(c,i,:)$, where I use ${\cal B}$ to denote $B \otimes B$.
\item ${\cal Z}(:,:,j) = {\hat{\cal G}}(:,:,j) {\cal W}(:,:,j)$
\item ${\cal O'}(n,i,:) = {\cal A}^T {\cal Z}(n,i,:)$, where I use ${\cal A}$ to denote $A \otimes A$.
\end{enumerate}

Now, the first part of the back propagation is to compute $\frac{\partial L}{\partial {\cal I'}}$ given
$\frac{\partial L}{\partial {\cal O'}}$. We will use the equations given in the previous section as follows.
\begin{enumerate}
\item $\frac{\partial L}{\partial {\cal Z}}(n,i,:) = {\cal A} \frac{\partial L}{\partial {\cal O'}}(n,i,:)$
\item Because ${\cal Z}(:,i,j) = {\hat{\cal G}}(:,:,j) {\cal W}(:,i,j)$, we have
      $$
      \frac{\partial L}{\partial {\cal W}}(:,i,j) = ({\hat{\cal G}}(:,:,j))^T \frac{\partial L}{\partial Z}(:,i,j)
      $$
      In other words,
      $$
      \frac{\partial L}{\partial {\cal W}}(:,:,j) = ({\hat{\cal G}}(:,:,j))^T \frac{\partial L}{\partial Z}(:,:,j)
      $$
\item $\frac{\partial L}{\partial {\cal I'}}(c,i,:) = {\cal B} \frac{\partial L}{\partial {\cal W}}(c,i,:)$
\end{enumerate}
These are the same as Equations 1, 2, and 4 of the very first section.


The other part of back propagation computes $\frac{\partial L}{\partial \hat{\cal G}}(n,c,j)$ for all
$n, c, j$. Here I arrive at something slightly different.

\begin{enumerate}
\item First compute $\frac{\partial L}{\partial {\cal Z}}$ ``column-by-column'' by
$$
\frac{\partial L}{\partial {\cal Z}}(n,i,:) = {\cal A} \frac{\partial L}{\partial O'}(n,i,:)
$$
This has been done previously. 
\item Next, given ${\cal Z}(:,:,j) = \hat{\cal G}(:,:,j) {\cal W}(:,:,j)$, we use the 2-dimensional equation (in the 
background section) and obtain
$$
\frac{\partial L}{\partial \hat{\cal G}}(:,:,j) = \frac{\partial L}{\partial {\cal Z}}(:,:,j) ({\cal W}(:,:,j))^T
$$
\end{enumerate}
In other words, this differs from Equation 3 of the very first section by a transposition. If one just check the dimension,
the multiplication without transposing ${\cal W}$ may not make sense.

\section{A Higher Level Question}
This layer starts from ${\cal I'}$ and produces ${\cal O'}$. Going back to a question I (Peter) raised earlier: can
this fit seamlessly into the rest of the network? I believe the output of one layer (the top) must be exactly the
same as the input (bottom) of the next layer. Note that in the time-domain code, the layer just prior to this Winograd
layer produces ${\cal I}$, not ${cal I'}$. Granted ${\cal I'}$ is determined exactly from ${\cal I}$, the number of
elements are not the same. That is, ${\cal I'}$ cannot be obtained by simple ``reshaping'' of ${\cal I}$.
So how can one just substitute the Winograd layer for the original time-domain layer?

The time-domain output ${\cal O}$ should be the same as the Winograd output ${\cal O'}$ except for some reshaping.

\newcommand{\tens}[1]{{\cal {{#1}}}}
To formally link $\tens{I'}$ back to $\tens{I}$, we can say the following. Any index $\mathbf{i'}$ for $\tens{I'}$
is linked to $\tens{I}$ via an index mapping $\phi$:
$$
\tens{I'}(\mathbf{i'}) = \tens{I}(\phi(\mathbf{i'})).
$$
Note that $\phi$ is a many-to-one mapping (does not have an inverse). 
In a layer that starts from $\tens{I}$ to $\tens{O'}$, one would need to compute $\frac{\partial L}{\partial \tens{I}}(\mathbf{i})$
where $\mathbf{i}$ are the indexes for $\tens{I}$. By chain rule
$$
\frac{\partial L}{\partial I}(\mathbf{i}) = 
\sum_{\mathbf{j'}} \frac{\partial L}{\partial \tens{I'}_{\mathbf{j'}}} \, \cdot \,
                   \frac{\partial \tens{I'}_{\mathbf{j'}}}{\partial \tens{I}_{\mathbf{i}}}
$$
But $\frac{\partial \tens{I'}_{\mathbf{j'}}}{\partial \tens{I}_{\mathbf{i}}}$ is either 0 or 1, and the value is 1 iff
$\phi(\mathbf{j'}) = \mathbf{i}$. 

$$
\frac{\partial L}{\partial I}(\mathbf{i}) = 
\sum_{\mathbf{j'} \in \phi^{-1}(\{\mathbf{i}\})} \frac{\partial L}{\partial \tens{I'}_{\mathbf{j'}}}.
$$


==> winograd_layer_define.tex <==
\section{Winograd Layers -- Definition}\label{sec:winograd_layer_define}

Consider a typical convolution layer where the input tensors with $C$ channels
of features maps each of dimension $H_i\times W_i$ are transformed into $K$
output channels via a simple unit-stride, unit-dilation linear
convolution with kernels of size $r\times s$:
\[
\tens{I}\in\reals^{C\times H_i \times W_i} \rightarrow
\tens{O}\in\reals^{K\times H_o \times W_o},
\]
$H_o = H_i-r+1$ and $W_o=W_i-s+1$, 
via
\begin{equation}\label{eqn:conv-std}
\tens{O}(k,:,:) = \sum_{c=1}^C \tens{W}(k,c,:,:) \conv \tens{I}(c,:,:)
\end{equation}
where $\conv$ stands for 2D linear convolution.


%To incorporate this layer Within a software framework, one implements the forward and backward passes.
%\jpark{Any reason "Within" is capitalized? Software framework $\rightarrow$ CNN framework? We may don't need the remainder of this paragraph.}
%The former computes $\tens{O}$
%given $\tens{I}$ and $\tens{W}$; the latter computes the partial derivatives of the
%scalar loss function $L$ with respect to $\tens{I}$ and $\tens{W}$ where the partial derivative
%of $L$ with respect to $\tens{O}$ and the current values of $\tens{I}$ and $\tens{W}$ are
%available.

The computation of Equation~\ref{eqn:conv-std} can be performed using the
Winograd transform which has a lower arithmetic complexity than Equation~\ref{eqn:conv-std}
suggests. The details of this computation
we present now are crucial to our definition of Winograd layers and their training.
First, the convolution $\tens{W}(k,c,:,:)\conv\tens{I}(c,:,:)$ can be broken down into
smaller tiles of $\tens{I}$ via an overlap procedure that is often used
in the context of digital signal processing.
We illustrate overlapping by the following one-dimensional example, using Matlab-like
array index notation that is self explanatory.
%\jpark{The overlap method may not be well-known to ICML folks. Mention that indices here follow the Matlab notation?}
\[
W(0:2) \conv I(0:5) \rightarrow O(0:3)
\]
can be computed as
\[
W(0:2) \conv
\left[\begin{array}{c} I(0:3) \\ I(2:5) \end{array}\right] \rightarrow
\left[\begin{array}{c} O(0:1) \\ O(2:3) \end{array}\right].
\]
Note that $I$ is broken up into two tiles with some duplicating elements while $O$ is partitioned
(without duplication) into two tiles. More generally, given convolution kernels of size $r\times s$
and (small) sizes $m, n$ that divide\footnote{
This assumption simplifies the presentation and can be easily eliminated by for example
zero padding.
}
$H_o$ and $W_o$, respectively,
we can reshape the input and output tensors $\tens{I}$, $\tens{O}$ into $\tilde{\tens{I}}$, $\tilde{\tens{O}}$
%\jpark{A picky reviewer may ask what happens if $H_o$ or $W_o$ is a prime. The tile size doesn't need
%to divide the image size. We can footnote we assume tile size divides image size for simplicity}:
\[
\tens{I}\in\reals^{C\times H_i\times W_i} \rightarrow
\tilde{\tens{I}}\in\reals^{C\times T\times (m+r-1)\times (n+s-1)}
\]
and
\[
\tens{O}\in\reals^{C\times H_o\times W_o} \rightarrow
\tilde{\tens{O}}\in\reals^{C\times T\times m\times n} .
\]
The value $T$ is the number of resulting tiles of the reshaping,
$T = H_o W_o / (mn)$. The input tile size is $(m+r-1)\times (n+s-1)$, while the output tile size is $m\times n$.
We express the reshaping by two index mapping functions $\phi$ and $\psi$
\[
\tilde{\tens{I}}(c,t,i,j) = \tens{I}(c,\phi(t,i,j)), \quad
\tens{O}(k,i,j) = \tilde{\tens{O}}(c,\psi(i,j))
\]
where $\phi$ is many-to-one and maps a 3-tuple to a 2-tuple while
$\psi$ is invertible and maps a 2-tuple to a 3-tuple.
Using the overlapped form, we have
\begin{equation}\label{eqn:conv-overlapped}
\tilde{\tens{O}}(k,t,:,:) =
\sum_{c=1}^C \tens{W}(k,c,:,:) \conv \tilde{\tens{I}}(c,t,:,:).
\end{equation}
Straightforward convolution of a $r\times s$ array $U$ with a
$(m+r-1)\times(n+s-1)$ array $V$ takes $mnrs$ multiplications. In contrast,
Winograd's method can possibly need only as few as
$(m+r-1)(n+s-1)$ multiplications via:%this is only for multiplication, addition is a different story.
\[
U\conv V =
A_1^T\left[
(G_1 U G_2^T) \odot (B_1^T V B_2)
\right] A_2.
\]
The six matrices $A_j, G_j, B_j$, $j=1,2$, (of consistent dimensions)
are independent of $U$ and $V$, and $\odot$ is element-wise multiplication. In
many instances the $A_j, B_j, C_j$ matrices are so simple that applying them requires
no multiplications. For example when $r=s=3$ and $m=n=2$, $A_1=A_2$, $B_1=B_2$
and $G_1=G_2$ and are respectively
\[
\left[
\begin{array}{c c}
1 & 0 \\ 1 & 1 \\ 1 & -1 \\ 0 & -1
\end{array}
\right],
\left[
\begin{array}{c c c c}
1 & 0 & 0 & 0 \\ 0 & 1 & -1 & 1 \\ -1 & 1 & 1 & 0 \\ 0 & 0 & 0 & -1
\end{array}
\right],
\left[
\begin{array}{c c c}
1 & 0 & 0 \\ \half & \half & \half \\ \half & -\half & \half \\ 0 & 0 & 1
\end{array}
\right].
\]
Thus, using tiling and Winograd transformation, Equation~\ref{eqn:conv-std} is
equivalent to
\begin{align}\label{eqn:conv-winograd}
\begin{split}
&\tilde{\tens{O}}(k,t,:,:) = \\
&A_1^T
\left[
\sum_{c=1}^C
\left(
G_1\tens{W}(k,c,:,:)G_2^T
\right)
\odot
\left(
B_1^T\tilde{\tens{I}}(c,t,:,:)B_2
\right)
\right]
A_2.
\end{split}
\end{align}
Motivated by this, we define a Winograd layer to be a topology
specified by a tensor
$\tens{W}_F \in \reals^{K\times C\times (m+r-1)\times (n+s-1)}$
that computes $\tens{O}$ from $\tens{I}$ via
\begin{align}\label{eqn:winograd_layer}
\begin{split}
& \tilde{\tens{I}}(c,t,i,j) = \tens{I}(c,\phi(t,i,j)), \\
& \tilde{\tens{O}}(k,t,:,:) = \\
& \phantom{k} A_1^T
\left[
\sum_{c=1}^C
\left(
\tens{W}_F(k,c,:,:)
\right)
\odot
\left(
B_1^T\tilde{\tens{I}}(c,t,:,:)B_2
\right)
\right]
A_2, \\
&\tens{O}(k,i,j) = \tilde{\tens{O}}(k,\psi(i,j))
\end{split}
\end{align}
Since $m, n >1$ in practice, $(m+r-1)(n+s-1) > rs$ and a
Winograd layer (Equation~\ref{eqn:winograd_layer}) has a higher
capacity than a corresponding convolution layer (Equation~\ref{eqn:conv-std}).





==> winograd_layer_implement.tex <==
\section{Winograd Layers -- Backward Propagation}\label{sec:winograd_layer_implement}

%\jpark{In the title of this section, implementation $\rightarrow$ backward propagation?}

To incorporate a Winograd layer within a standard CNN framework (e.g. Caffe) so as to
allow training and inference, it suffices to be able to compute the forward and backward passes.
The forward pass is straightforward as it simply follows
Equation~\ref{eqn:winograd_layer}, for which we note that~\cite{winograd}
details an optimized implementation.
For the backward pass, we need to compute the partial derivatives of the
scalar loss function $L$
w.r.t. each of the variables $\tens{I}(c,i,j)$ and $\tens{W}_F(k,c,i,j)$ in terms of the
known partial derivatives of $L$ w.r.t. $\tens{O}(k,i,j)$, or $\partial L/\partial \tens{O}$
in short. We present the derivations here as they pertain to the Winograd layers
and are thus unavailable elsewhere.\footnote{Note that the Winograd-kernel approach~\cite{winograd} simply uses Winograd to accelerate the convolution operations in both forward and backward propagation (with proper adjustments when accelerating backward propagation) and does not consider Winograd as a layer architecture with full fledged backward propagation.}

First, we use this key form of chain rule: Suppose the partial derivatives of a scalar function
$L$ w.r.t. an array of variables $y_{ij}$, $Y\in\reals^{\mu\times\nu}$, are known. Moreover,
the variables $Y$ are in fact dependent variables of an array of variables $x_{ij}$,
$X\in\reals^{\mu'\times\nu'}$ via $Y = U^T X V$ where $U, V$ are constant matrices
of commensurate dimensions. The partial derivatives of $L$ w.r.t. $X$ are then given by
\begin{equation}\label{eqn:chain_rule}
\frac{\partial L}{\partial X} =
U  \frac{\partial L}{\partial Y}  V^T.
\end{equation}

Next, introduce intermediate tensors  $\tilde{\tens{I}}_F$ and $\tens{Z}$
\begin{align}\label{eqn:aux_tensors}
\begin{split}
\tilde{\tens{I}}_F(c,t,:,:) &= B_1^T\,\tilde{\tens{I}}(c,t,:,:)\,B_2, \\
\tens{Z}(k,t,:,:) &= \sum_{c=1}^C \tens{W}_F(k,c,:,:)\odot\tilde{\tens{I}}_F(c,t,:,:), \\
\tilde{\tens{O}}(k,t,:,:) &= A_1^T\,\tens{Z}(k,t,:,:)\,A_2,
\end{split}
\end{align}
for all applicable indices $c, k, t$.

To obtain $\partial L/\partial \tens{W}_F$, apply Equation~\ref{eqn:chain_rule}
(the Chain Rule) while noting from Equation~\ref{eqn:aux_tensors} that the first two
dimensions of $\tens{Z}$ are in fact the product of two matrices:
\begin{equation}\label{eqn:matrix_product_form}
\tens{Z}(:,:,i,j) = \tens{W}_F(:,:,i,j) \tilde{\tens{I}}_F(:,:,i,j),
\end{equation}
for all fixed and applicable $i$ and $j$. Hence,
\begin{align}\label{eqn:partial_L_partial_WF}
\begin{split}
\frac{\partial L}{\partial \tilde{\tens{O}}(k,t,i,j)}
&=
\frac{\partial L}{\partial \tens{O}(k,\psi^{-1}(t,i,j))}, \\
\frac{\partial L}{\partial \tens{Z}(k,t,:.:)}
&=
A_1\,\frac{\partial L}{\partial \tilde{\tens{O}}(k,t,:,:)}\,A_2^T, \\
\frac{\partial L}{\partial \tens{W}_F(:,:,i,j)}
&=
\frac{\partial L}{\partial \tens{Z}(:,:,i,j)}\,
\left(\tilde{\tens{I}}_F(:,:,i,j)\right)^T.
\end{split}
\end{align}
Note that the last equality above depends on Equation~\ref{eqn:matrix_product_form},
and the transposition applies to the first two dimensions of
$\tilde{\tens{I}}_F$.

Similarly, we use the Chain Rule to obtain $\partial L/\partial \tens{I}$, noting
that $\partial L/\partial \tens{Z}$ is already computed previously:
\begin{align}\label{eqn:partial_L_partial_I}
\begin{split}
\frac{\partial L}{\partial \tilde{\tens{I}}_F(:,:,i,j)}
&=
\left(\tens{W}_F(:,:,i,j)\right)^T\,\frac{\partial L}{\partial \tens{Z}(:,:,i,j)}, \\
\frac{\partial L}{\partial \tilde{I}(c,t,:,:)}
&=
B_1\,\frac{\partial L}{\partial \tilde{\tens{I}}_F(c,t,:,:)}\,B_2^T, \\
\frac{\partial L}{\partial \tens{I}(c,i,j)}
&=
\sum_{\substack{t,i',j'\;\text{where} \\\ (i,j) = \phi(t,i',j')}}
\frac{\partial L}{\partial \tilde{\tens{I}}(c,t,i',j')}.
\end{split}
\end{align}
In summary, the backward propagation of Winograd layers is implemented by Equations~\ref{eqn:partial_L_partial_WF}
and~\ref{eqn:partial_L_partial_I}.
%Most of these operations can take advantage of highly optimized BLAS level-3 routines as will be shown in our public code repository at https://github.com/IntelLabs/SkimCaffe ({\tt intel\_sparse\_winograd} branch).


==> winograd_layer_sparsify_old.tex <==
\section{Winograd Layers -- Training and Pruning}
\label{sec:winograd_layer_sparsify}

Consider now a $L$-layer network with a mixture of layers such as
convolution, Winograd, fully connected, and pooling. Denote the
parameters by the vector
$\btheta = [\mathbf{w}_{(1)},\mathbf{w}_{(2)},\ldots,\mathbf{w}_{(L)}]$
where the subscripts correspond to the layer number.
For a given loss function, a standard Stochastic Gradient Descent
training updates the parameters via $
{\btheta}^{(k+1)} =
{\btheta}^{(k)} - \eta_k \, \nabla_{\cal B} E(\btheta).
$
The overall goal
here is to arrive at a $\btheta^*$ such that many of its elements, including
those within the Winograd layer, are zero.
%of pruning such network is to obtained trained parameters, $\btheta^*$ such that many of
%the coefficients, including those within the Winograd layers, are zero. This paper focuses on pruning %Winograd coefficients.
Pre-training, pruning, and fine-tuning (re-training) are the three major steps
that help us toward this goal. More specifically, each step described below
consists of critical techniques that improve sparsity, accuracy, and efficiency.

%Several techniques are involved:
%(1) initialization by pre-training,
%(2) pruning with regularization and gradient-based thresholding, and
%(3) fine-tuning (re-training)

\subsection{Pre-training: Implications of Domain Selection}
The main goal of the pre-training step is to train the neural network to achieve a high accuracy to be used as the starting point for the pruning step. Previously, this
pre-training step is done in the spatial convolution domain.
With our newly defined Winograd convolution layer,
we have the additional option to perform this step directly in Winograd domain.

\paragraph*{Pre-train in Winograd Domain:}

With Winograd convolution layers, pre-training directly in Winograd domain is straightforward and has an advantage of potentially
getting higher accuracy as shown in Section~\ref{subsec:sparsity_accuracy} because a Winograd convolution layer has capacity larger than the corresponding spatial convolution layer\footnote{Although not a focus of this paper, we obtain an accuracy higher than the original AlexNet (58.0\% vs. 57.4\%) when we train directly in Winograd domain to get the pre-trained model.}
%This indicates a potential of achieving higher accuracies due to capacity larger than spatial convolution layers.}. %Indeed, by pre-training directly in Winograd domain, we have achieved 58\% top-1 accuracy on AlexNet, a 0.5\% improvement than the top-1 accuracy obtained by pre-training in the spatial domain.

\paragraph*{Pre-train in Spatial Domain:}

Pre-training in spatial domain also has its own advantage. Particularly, many networks have models pre-trained in spatial domain available, which can save time. However, because of the domain shift from spatial to Winograd, a \emph{smoother} is needed to pre-process the spatial domain models before applying both regularization and thresholding in Winograd domain in the pruning step.
Particularly, the smoother further trains the models with a regularization function $R$ applied to the Winograd parameters, which are computed ``on-the-fly'' based on the $G_j$ matrices in Equation~\ref{eqn:conv-winograd}: $
E(\btheta) = L(\btheta) + \lambda R( G(\btheta) ),
$
where $G(\btheta)$ transforms those spatial convolution parameters into the Winograd representation, while leaving others unchanged.
The smoother produces $\btheta^*$, when finishing pre-processing. Then, we start the pruning step with
Winograd layers as below using $\btheta^{({\rm start})} \leftarrow G(\btheta^*)$.
%We observe that this smoother is useful when using pre-trained spatial domain models to save pre-training time.

%Given a network with both standard convolution as well as Winograd layers\footnote{because of differen kernel sizes in different convolution layers, one can choose the best convolution algorithm for each layer. Thus, it is possible that both spatial convolution layers and Winograd layers are used in the network}, one can employ
%common initialization schemes such as random numbers with Gaussian distributions. Training of such network
%
%
%Alternatively, even if we aim at employing Winograd layers, we can start with a network with
%convolution layers in place of the Winograd layers. In this case
%we train with a regularization function (more on this later)
%applied to the Winograd parameters, which are computed ``on-the-fly'' based on the
%$G_j$ matrices in Equation~\ref{eqn:conv-winograd}:
%\[
%E(\btheta) = L(\btheta) + \lambda R( G(\btheta) )
%\]
%where $G(\btheta)$ transforms into the Winograd representation
%those convolution kernels that are meant
%to be implemented using the Winograd method, while leaving others unchanged.
%When this pre-training phase is finished, producing $\btheta^*$,
%we start the training with
%Winograd layers using $\btheta^{({\rm start})} \leftarrow G(\btheta^*)$.

\subsection{Pruning with Regularization and Gradient-based Thresholding}
\label{pruning}
Pruning is always done directly in Winograd domain, which is enabled by the Winograd layer. Regularization and gradient-based thresholding are the two techniques used for pruning. Regularization is a common and useful technique to attenuate over-fitting and induce sparsity.
In common frameworks such as Caffe, one can easily incorporate different regularization
functions on different layers. In essence, one minimizes the
energy function of the form
\begin{equation}\label{eqn:energy_function}
E(\btheta) = L(\btheta) + R(\btheta),
\;
R(\btheta) = \sum_{\ell=1}^L \lambda_\ell \| \mathbf{w}_{(\ell)}\|_{p_\ell}.
\end{equation}
Common choices of norms are $p_{\ell}=1$ or $2$, and we use $L1$-norm for the layers to prune.
%
%\jpark{We may don't need the following 2 sentences. Anyway, I guess this section needs to be modified because now we're describing Winograd layer as a new CNN architecture?}
%Given a loss function $L$ that only encapsulates how closely a network produce the expected
%answer, one often adds to it a regularization term on the parameters. Training of the network
%entails minimizing the sum of the loss function and the regularization terms.
%We employ a regularization that can target the Winograd and non-Winograd differently, and
%the function we aim to minimize during training is of the form
%\begin{equation}\label{eqn:energy_functionnn}
%E(\btheta) = L(\btheta) + \lambda_1 R_1( \mathbf{w}_F ) + \lambda_2 R_2( \mathbf{w} ).
%\end{equation}
%where $R_1$ and $R_2$ are two regularization functions. In general, we use the $\ell_1$
%and $\ell_2$ norms for $R_1$ and $R_2$, respectively. The numbers $\lambda_1$ and
%$\lambda_2$ are considered hyper-parameters. Note that the gradients of $R_1$ and $R_2$
%are both straightforward and economical to compute.

%\subsection*{Gradient-based Thresholding}
To achieve higher sparsity, thresholding is used in addition to regularization.
The idea of thresholding is to set to zero particular
entries within the parameter $\btheta^{(k)}$ that are deemed inconsequential~\citep{prune,sscnn,dns}.
Instead of using one uniform threshold to judge the significance of all parameters, the threshold
on a particular parameter is dependent on how significantly this parameter affects
the underlying loss function $L$. The thresholding function
$T_{\epsilon,\beta}$ is of the form
\begin{equation}\label{eqn:thresholding_function}
T_{\epsilon,\beta}( w ) =
\left\{
\begin{array}{l l}
0 & \mbox{if $|w|\left(|\frac{\partial L}{\partial w}(\btheta)|+\beta \right) < \epsilon$} \\
w & \mbox{otherwise}
\end{array}.
\right.
\end{equation}
We apply the thresholding function to a vector simply by applying it
on each element, denoted with the slightly abused notation: $T_{\epsilon,\beta}(\mathbf{w})$.
The numbers $\epsilon$ and $\beta$ are part of the ``hyper-parameters'' of the training procedure.
This scheme uses smaller thresholds as the magnitude of gradient increases (threshold is $\epsilon/\beta$, $\epsilon$, and 0, when the magnitude
of gradient is 0, $1 - \beta$, and $\infty$, respectively).
We find that the choice of $\epsilon$=1e-4 and $\beta$=0.1 works well.
We emphasize that thresholding the parameters including Winograd parameters is now straightforward
because of the Winograd parameters are the direct independent parameters of the Winograd layers.

In the Winograd domain, where the L-layer network contains both Winograd layers and other layers (e.g., pooling) with parameters: $\btheta = [\mathbf{w}_{(1)},\ldots,\mathbf{w}_{(L)}]$, the pruning step applies regularization and thresholding as the following:
{\setlength{\mathindent}{-0.2cm}\begin{equation}\label{eqn:winograd_training_1}
\begin{split}
E(\btheta)
= L(\btheta) + \sum_{\ell=1}^L \lambda_\ell \|\mathbf{w}_{(\ell)}\|_{p_\ell}, \quad
\btheta^{({\rm tmp})}
\leftarrow
\btheta^{(k)} - \eta_k \nabla_{\cal B} E(\btheta^{(k)}), \quad
\btheta^{(k+1)}
\leftarrow T_{\epsilon,\beta}( \btheta^{({\rm tmp})} ).
\end{split}
\end{equation}}


%The procedure is:
%\begin{enumerate}
%\item Obtain $\btheta^{({\rm start})}$ using the training without Winograd layers.
%\item Switch to Winograd layers and thus the parameters now consist of Winograd
%      and non-Winograd parts: $\btheta = [\mathbf{w}_{(1)},\ldots,\mathbf{w}_{(L)}]$.
%      Train with regularization and thresholding:
%\begin{align}\label{eqn:winograd_training_1}
%\begin{split}
%E(\btheta)
%&= L(\btheta) + \sum_{\ell=1}^L \lambda_\ell \|\mathbf{w}_{(\ell)}\|_{p_\ell},\\
%\btheta^{({\rm tmp})}
%&\leftarrow
%\btheta^{(k)} - \eta_k \nabla_{\cal B} E(\btheta^{(k)}), \\
%\btheta^{(k+1)}
%&\leftarrow T_{\epsilon,\beta}( \btheta^{({\rm tmp})} ).
%\end{split}
%\end{align}
%\end{enumerate}

%We find some Winograd parameters have larger values and derivatives during pruning. We believe this is because the transformation matrices $G_1$ and $G_2$ do not have unit row norms. Therefore, smaller learning rates for Winograd layers need to be used in the subsequent steps. %Alternatively, a model with batch normalization layers~\cite{ioffe2015batch} can also mitigate this problem.

\subsection{Fine-Tuning: Recover Accuracy Loss}
\label{fine_tuning}
Similar to pruning in spatial domain, pruning Winograd parameters will cause accuracy loss,
which necessitates a fine-tuning step to recover the loss.
Same as pruning, fine-tuning is only done in the Winograd domain. During fine-tuning, the zero parameters obtained from the pruning step are fixed, while the network is trained to adjust the other non-zeros parameters to recover accuracy loss. We use L2 regularization during fine-tuning.
%Since we want to achieve high sparsity without accuracy loss, we need to be careful with the delicate tradeoff between sparsity and accuracy loss in the pruning step. Fortunately,
The larger capacity of Winograd domain gives another benefit here. Even with a high sparsity, the Winograd domain still retains more Winograd parameters due to its larger capacity than its spatial counterpart. Therefore, fine-tuning in Winograd domain can be more resilient to high sparsity while maintaining accuracy, so we can use regularization and thresholding more aggressively during pruning.
%and let the fine-tuning step to recover the accuracy loss.
%And our experiments indeed verify this hypothesis.




